Hierarchical clustering and the baryon distribution in galaxy clusters

The baryon fraction of galaxy clusters in numerical simulations is found to be dependant on the cluster formation method. In all cases, the gas is anti-biased compared with the dark matter. However, clusters formed hierarchically are found to be more depleted in baryons than clusters formed non-hierarchically. There is a depletion of 10 to 15% for hierarchically formed clusters while the depletion is less than 10% for those clusters formed non-hierarchically. This difference is dependent on the mass of the clusters. The mean baryon enrichment profile for the hierarchically formed clusters shows an appreciable baryon enhancement around the virial radius not seen in the clusters formed without substructure. If this phenomenon applies to real clusters, it implies that determinations of the baryon fractions in clusters of galaxies require data extending beyond the virial radius of the clusters in order to achieve an unbiased value.

==> Makefile <==
DOC=main

$(DOC).ps: $(DOC).dvi
	dvips $(DOC) -o

$(DOC).dvi: $(DOC).bbl
	RERUN=1;\
        while(test $${RERUN} -ge 1); do \
         RERUN=`latex $(DOC).tex | grep Rerun | wc | awk '{print $$1}'`; \
        done
	-latex $(DOC).tex | grep Warning

$(DOC).bbl: $(DOC).aux biblio.bib $(DOC).tex
	bibtex $(DOC)

$(DOC).aux: $(DOC).tex
	latex $(DOC).tex

clean:
	-rm $(DOC).bbl $(DOC).blg
	-find . \( -name "*.dvi" -o -name "*.log" -o \
                   -name "*.aux" -o -name "*.ps" -o  \
                   -name "*.bak" \) -exec rm {} \;

spell:
	find . -name "*.tex" -exec ispell -t {} \;
	find . -name "*.tex" -exec grep -l -i recognis {} \;
	find . -name "*.tex" -exec grep -l -i criticis {} \;
	find . -name "*.tex" -exec grep -l -i emphasis {} \;
	find . -name "*.tex" -exec grep -l -i organis {} \;
	find . -name "*.tex" -exec grep -l -i parametris {} \;
	find . -name "*.tex" -exec grep -l -i halos {} \;
	find . -name "*.tex" -exec grep -l -i best-fit {} \;
	find . -name "*.tex" -exec grep -l -i disk {} \;
	find . -name "*.tex" -exec grep -l -i nonlinear {} \;
	find . -name "*.tex" -exec grep -l -i onto {} \;
	find . -name "*.tex" -exec grep -l -i timescale {} \;

# This checks the .eps figures for PS operators that are not allowed
# in submissions to ApJ
check_figs:
	-grep -l banddevice     Figures/figs/*.eps
	-grep -l clear          Figures/figs/*.eps
	-grep -l cleardictstack Figures/figs/*.eps
	-grep -l copypage       Figures/figs/*.eps
	-grep -l erasepage      Figures/figs/*.eps
	-grep -l exitserver     Figures/figs/*.eps
	-grep -l framedevice    Figures/figs/*.eps
	-grep -l grestoreall    Figures/figs/*.eps
	-grep -l initclip       Figures/figs/*.eps
	-grep -l initgraphics   Figures/figs/*.eps
	-grep -l initmatrix     Figures/figs/*.eps
	-grep -l quit           Figures/figs/*.eps
	-grep -l renderbands    Figures/figs/*.eps
	-grep -l setglobal      Figures/figs/*.eps
	-grep -l setpagedevice  Figures/figs/*.eps
	-grep -l setshared      Figures/figs/*.eps
	-grep -l startjob       Figures/figs/*.eps

check_doubles:
	find . -name "*.tex" -exec grep -l "of of" {} \;
	find . -name "*.tex" -exec grep -l "the the" {} \;

#depend:
#	-rm depend
#	tex_depend $(DOC).tex

#include depend

